Complex diffusion-based kinetics of photoluminescence in semiconductor nanoplatelets

We present a diffusion-based simulation and theoretical models for explanation of photoluminescence (PL) emission intensity in semiconductor nanoplatelets. It is shown that the shape of PL intensity curves can be reproduced by the interplay of recombination, diffusion and trapping of excitons. The emission intensity at short times is purely exponential and is defined by recombination. At long times it is governed by the release of excitons from surface traps and is characterized by a power-law tail. We show that the crossover from one limit to another is controlled by diffusion properties. This intermediate region exhibits a rich behaviour depending on the value of diffusivity. Proposed approach reproduces all the features of experimental curves measured for different nanoplatelet systems.

==> literature.tex <==
@BOOK{Ivchenko,
  title = {{O}ptical spectroscopy of semiconductor nanostructures},
  publisher = {Alpha Science Int.},
  year = {2005},
  author = {Ivchenko, E .L.},
  address = {Harrow, UK}
 
}


@ARTICLE{Saidzhonov,
  author = {Saidzhonov, B.M. and Kozlovsky, V.F. and Zaytsev, V.B. and Vasiliev, R.B.},
  title = {Ultrathin CdSe/CdS and CdSe/ZnS core-shell nanoplatelets: The impact of the shell material on the structure and optical properties},
  journal = {Journal of Luminescence},
  year = {2019},
  volume = {209},
  pages = {170},
  doi = {10.1016/j.jlumin.2019.01.052}
}

@ARTICLE{Erdem,
  author = {Erdem, T. and Demir, H.V.},
  title = {Colloidal nanocrystals for quality lighting and displays: milestones and recent developments},
  journal = {Nanophotonics},
  year = {2016},
  volume = {5},
  pages = {74},
  doi = {10.1515/nanoph-2016-0009}
}

@ARTICLE{Zaytsev,
  author = {Saidzhonov, B.M. and Zaytsev, V.B. and Berekchiian, M.V. and Vasiliev, R.B.},
  title = {Highly luminescent copper-doped ultrathin CdSe nanoplatelets for white-light generation},
  journal = {Journal of Luminescence},
  year = {2020},
  volume = {222},
  pages = {117134},
  doi = {10.1016/j.jlumin.2020.117134}
}

@ARTICLE{Achtstein2,
  author = {Achtstein, A.W. and Marquardt, O. and Scott, R. and Ibrahim, M. and Riedl, T. and Prudnikau, A.V. and Antanovich, A. and Owschimikow, N. and Lindner, J.K.N. and Artemyev, M. and Woggon, U.},
  title = {Impact of shell growth on recombination dynamics and exciton-phonon interaction in CdSe-CdS core-shell nanoplatelets},
  journal = {ACS Nano},
  year = {2018},
  volume = {12},
  pages = {9476},
  doi = {10.1021/acsnano.8b04803}
}

@ARTICLE{Scott,
  author = {Scott, R. and Kickh\"ofel, S. and Schoeps, O. and Antanovich, A. and Prudnikau, A. and Chuvilin, A. and Woggon, U. and Artemyev, M. and Achtstein, A.W.},
  title = {Temperature dependent radiative and nonradiative recombination dynamics in CdSe–CdTe and CdTe–CdSe type II hetero nanoplatelets},
  journal = {Phys. Chem. Chem. Phys.},
  year = {2016},
  volume = {18},
  pages = {3197},
  doi = {10.1039/C5CP06623A}
}


@ARTICLE{Colvin,
  author = {Colvin, V. L. and Schlamp, M. C.  and Alivisatos, A. P.},
  title = {{L}ight-emitting diodes made from cadmium selenide nanocrystals and a semiconducting polymer},
  journal = {Nature},
  year = {1994},
  volume = {370},
  pages = {354--357},
  doi = {10.1038/370354a0}
}


@ARTICLE{Klimov,
  author = {Klimov, V. I. and  Mikhailovsky, A. A. and Xu, S. and Malko, A. and Hollingsworth, J. A.  and Leatherdale, C. A. and Eisler, H. J. and Bawendi, M. G.},
  title = { {O}ptical gain and stimulated emission in nanocrystal quantum dots},
  journal = {Science},
  year = {2000},
  volume = {290},
  pages = {314--317},
  doi = {10.1126/science.290.5490.314}
}


@ARTICLE{Nazzal,
  author = {Nazzal, Amjad Y. and Qu, Lianhua  and Peng, Xiaogang and Xiao, Min},
  title = { {P}hotoactivated {C}d{S}e {N}anocrystals as {N}anosensors for {G}ases},
  journal = {Nano Lett.},
  year = {2003},
  volume = {3},
  issue = {6},
  pages = {819--822},
  doi = {10.1021/nl0340935}
}


@ARTICLE{Xu,
  author = {Xu, Mingsheng and Liang, Tao  and Shi, Minmin and Chen, Hongzheng},
  title = { {G}raphene-{L}ike {T}wo-{D}imensional {M}aterials},
  journal = {Chem. Reviews},
  year = {2013},
  volume = {113},
  issue = {5},
  pages = {3766--3798},
  doi = {10.1021/cr300263a}
}


@ARTICLE{Ithurria,
  author = {Ithurria, Sandrine and Dubertret, Benoit},
  title = {{Q}uasi 2{D} {C}olloidal {C}d{S}e {P}atelets with {T}hicknesses {C}ontrolled at the {A}tomic Level},
  journal = {J. Am. Chem. Soc.},
  year = {2008},
  volume = {130},
  issue = {49},
  pages = {16504--16505},
  doi = {10.1021/ja807724e}
}


@article{PhysRevB.89.035307,
   author = {Benchamekh, R. and Gippius, N. A. and Even, J. and Nestoklon, M. O. and Jancu, J.-M. and Ithurria, S. and Dubertret, B. and Efros, Al. L. and Voisin, P.},
 title = {{T}ight-binding calculations of image-charge effects in colloidal nanoscale platelets of CdSe}, 
 journal = {Phys. Rev. B},
  volume = {89},
  issue = {3},
  pages = {035307},
  numpages = {7},
  year = {2014},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.035307}
 }


@ARTICLE{Grim,
  author = { Grim, J. Q. and Christodoulou, S. and Stasio, F. Di and Krahne, R. and Cingolani, R. and Manna, L. and Moreels, I.},
  title = {{C}ontinuous-wave {B}iexciton {L}asing at {R}oom {T}emperature {U}sing {S}olution-{P}rocessed {Q}uantum {W}ells},
  journal = {Nat. Nanotech.},
  year = {2014},
  volume = {9},
  pages = {891-5},
  doi = {10.1038/nnano.2014.213}
}



@ARTICLE{Achtstein,
  author = {Achtstein,  A. W. and Schliwa, A. and  Prudnikau, A. and Hardzei, M. and Artemyev, M. V. and Thomsen, C. and Woggon, U.},
  title = {{E}lectronic {S}tructure and {E}xciton-{P}honon {I}nteraction in {T}wo-{D}imensional {C}olloidal {C}d{S}e {N}anosheets},
  journal = {Nano Lett.},
  year = {2012},
  volume = {12},
  issue = {6},
  pages = {3151-3157},
  doi = {10.1021/nl301071n}
}


@ARTICLE{Ithurria_2,
  author = {Ithurria, S. and Tessier, M. D. and Mahler, B. and Lobo, R. P. and Dubertret, B. and Efros, A. L. },
  title = {{C}olloidal nanoplatelets with two-dimensional electronic structure},
  journal = {Nature Mater.},
  year = {2011},
  volume = {10},
  issue = {12},
  pages = {936-941},
  doi = {10.1038/nmat3145}
}



@ARTICLE{Mahler_1,
  author = {Mahler, Benoit and Nadal, Brice and Bouet, Cecile and Patriarche, Gilles and Dubertret, Benoit},
  title = {{C}ore/{S}hell {C}olloidal {S}emiconductor {N}anoplatelets},
  journal = {J. Am. Chem. Soc.},
  year = {2012},
  volume = {134},
  issue = {45},
  pages = {18591-18598},
  doi = {10.1021/ja307944d}
}


@ARTICLE{Tessier,
  author = {Tessier, M. D. and Spinicelli, P. and Dupont, D. and Patriarche, G. and Ithurria, S. and Dubertret, B.},
  title = {{E}fficient exciton concentrators built from colloidal core/crown CdSe/CdS semiconductor nanoplatelets},
  journal = {Nano Lett.},
  year = {2014},
  volume = {14},
  issue = {1},
  pages = {207-213},
  doi = {10.1021/nl403746p}
}


@ARTICLE{Biadala,
  author = {Biadala, L. and Liu, F. and Tessier, M. D. and Yakovlev, D. R. and Dubertret, B. and Bayer, M.},
  title = {{R}ecombination dynamics of band edge excitons in quasi-two-dimensional {C}d{S}e nanoplatelets},
  journal = {Nano Lett.},
  year = {2014},
  volume = {14},
  issue = {3},
  pages = {1134-1139},
  doi = {10.1021/nl403311n}
}


@ARTICLE{Pelton,
  author = {Pelton, M. and Ithurria, S. and Schaller, R.D. and Dolzhnikov, D.S. and Talapin, D. V.},
  title = {{C}arrier cooling in colloidal quantum wells},
  journal = {Nano Lett.},
  year = {2012},
  volume = {12},
  issue = {12},
  pages = {6158-6163},
  doi = {10.1021/nl302986y}
}


@ARTICLE{She,
  author = {She, C. and Fedin, I. and Dolzhnikov, D. S. and  Demortiere, A. and Schaller,  R. D. and Pelton, M. and Talapin, D. V.},
  title = {{L}ow-threshold stimulated emission using colloidal quantum wells},
  journal = {Nano Lett.},
  year = {2014},
  volume = {14},
  issue = {5},
  pages = {2772-2777},
  doi = {10.1021/nl500775p}
}


@ARTICLE{Guzelturk,
  author = {Guzelturk, Burak and Kelestemur, Yusuf and Olutas, Murat and Delikanli, Savas and Schaller,  Demir, Hilmi Volkan},
  title = {{A}mplified {S}pontaneous {E}mission and {L}asing in {C}olloidal {N}anoplatelets},
  journal = {ACS Nano},
  year = {2014},
  volume = {8},
  issue = {7},
  pages = {6599-6605},
  doi = {10.1021/nn5022296}
}

@ARTICLE{Bruchez,
  author = {Bruchez, M. Jr. and Moronne, M. and Gin, P. and Weiss, S. and Alivisatos, A. P.},
  title = {{S}emiconductor nanocrystals as fluorescent biological labels},
  journal = {Science},
  year = {1998},
  volume = {281},
  pages = {2013-2016},
  doi = {10.1126/science.281.5385.2013}
}


@ARTICLE{Manna,
  author = {Manna, Liberato and Milliron, Delia J. and Meisel, Andreas and Scher, Erik C. and Alivisatos, A. Paul},
  title = {{C}ontrolled growth of tetrapod-branched inorganic nanocrystals},
  journal = {Nature Materials},
  year = {2003},
  volume = {2},
  issue = {6},
  pages = {382-385},
  doi = {10.1038/nmat902}
}


@ARTICLE{Murray,
  author = {Murray, C. B. and Norris, D. J. and Bawendi, M. G.},
  title = {{S}ynthesis and characterization of nearly monodisperse {C}d{E} ({E} = sulfur, selenium, tellurium) semiconductor nanocrystallites},
  journal = {J. Am. Chem. Soc.},
  year = {1993},
  volume = {115},
  issue = {19},
  pages = {8706-8715},
  doi = {10.1021/ja00072a025}
}



@article {Michalet,
author = {Michalet, X. and Pinaud, F. F. and Bentolila, L. A. and Tsay, J. M. and Doose, S. and Li, J. J. and Sundaresan, G. and Wu, A. M. and Gambhir, S. S. and Weiss, S.},
title = {{Q}uantum {D}ots for {L}ive {C}ells, in {V}ivo {I}maging, and {D}iagnostics},
journal = {Science},
 volume = {307},
number = {5709},
pages = {538--544},
year = {2005},
doi = {10.1126/science.1104274}
		
}


@ARTICLE{Smirnov,
 author = {Smirnov, A.~M. and Golinskaya, A.~D. and Kotin, P.~A. and Dorofeev, S.~G. and Palyulin, V.~V. and Mantsevich, V.~N. and Dneprovskii, V.~S.},
 title = {{P}hotoluminescence and nonlinear transmission of {C}u-doped {C}d{S}e quantum dots},
 journal = {Journal of Luminescence},
 year = {2019},
 volume = {213},
 pages = {29-35},
 doi = {10.1016/j.jlumin.2019.05.001}
}


@ARTICLE{Smirnov_1,
 author = {Smirnov, Aleksandr M. and Golinskaya, Anastasiya D. and Kotin, Pavel A. and Dorofeev, Sergey G. and Zharkova, Ekaterina V. and Palyulin, Vladimir V.
 and Mantsevich, Vladimir N.  and Dneprovskii, Vladimir S.},
 title = {{D}amping of {C}u-{A}ssociated {P}hotoluminescence and {F}ormation of {I}nduced {A}bsorption in {H}eavily {C}u-{D}oped {C}d{S}e {Q}uantum {D}ots},
 journal = {J. Phys. Chem. C},
 year = {2019},
 volume = {123},
 issue = {45},
 pages = {27986-27992},
 doi = {10.1021/acs.jpcc.9b09918}
}



@ARTICLE{Nasilowski,
 author = {Nasilowski, Michel and Mahler, Benoit and Lhuillier, Emmanuel and Ithurria, Sandrine and Dubertret, Benoit},
 title = {{T}wo-{D}imensional {C}olloidal {N}anocrystals},
 journal = {Chem. Rev.},
 year = {2016},
 volume = {116},
 issue = {18},
 pages = {10934-10982},
 doi = {10.1021/acs.chemrev.6b00164}
}


@article {Owen,
author = {Owen, Jonathan},
title = {{T}he coordination chemistry of nanocrystal surfaces},
journal = {Science},
volume = {347},
issue = {6222},
pages = {615--616},
year = {2015},
doi = {10.1126/science.1259924}
		
}


@article {Boles,
author = {Boles, M. A. and Ling, D. and Hyeon, T. and Talapin, D. V.},
title = {{T}he surface science of nanocrystals},
journal = {Nat Mater.},
volume = {15},
issue = {2},
pages = {141--153},
year = {2016},
doi = {10.1038/nmat4526}
		
}



@article {Owen_1,
author = {Owen, Jonathan and Brus, Louis},
title = {{C}hemical {S}ynthesis and {L}uminescence {A}pplications of {C}olloidal {S}emiconductor {Q}uantum {D}ots},
journal = {J. Am. Chem. Soc.},
volume = {139},
issue = {32},
pages = {10939--10943},
year = {2017},
doi = {10.1021/jacs.7b05267}
		
}


@article {Shornikova,
author = {Biadala, Louis and Shornikova, Elena V. and Rodina, Anna V. and Yakovlev, Dmitri R. and Siebers, Benjamin and Aubert, Tangi and Nasilowski, Michel and Hens, Zeger and Dubertret, Benoit and Efros, Alexander L. and Bayer, Manfred },
title = {{M}agnetic polaron on dangling-bond spins in {C}d{S}e colloidal nanocrystals},
journal = {Nature Nanotechnology},	
volume = {12},
issue = {6},
pages = {569--574},
year = {2017},
doi = {10.1038/nnano.2017.22}
		
}


@article {Nirmal,
author = {Nirmal, M. and Dabbousi, B. O. and Bawendi, M. G. and Macklin, J. J. and Trautman, J. K. and Harris, T. D. and Brus, L. E.},
title = {{F}luorescence intermittency in single cadmium selenide nanocrystals},
journal = {Nature},	
volume = {383},
issue = {6603},
pages = {802--802},
year = {1996},
doi = {10.1038/383802a0}
		
}



@article{Banin,
author = {Banin,U.  and Bruchez,M.  and Alivisatos,A. P.  and Ha,T.  and Weiss,S.  and Chemla,D. S. },
title = {{E}vidence for a thermal contribution to emission intermittency in single {C}d{S}e/{C}d{S} core/shell nanocrystals},
journal = {The Journal of Chemical Physics},
volume = {110},
number = {2},
pages = {1195-1201},
year = {1999},
doi = {10.1063/1.478161}
}



@article{Kuno,
author = {Kuno,M.  and Fromm,D. P.  and Hamann,H. F.  and Gallagher,A.  and Nesbitt,D. J. },
title = {“{O}n”/“off” fluorescence intermittency of single semiconductor quantum dots},
journal = {The Journal of Chemical Physics},
volume = {115},
number = {2},
pages = {1028-1040},
year = {2001},
doi = {10.1063/1.1377883}

}


@article{Eli,
author = {Stefani, F. D.  and Hoogenboom,  J. P. and Barkai, E. },
title = {{B}eyond quantum jumps: {B}linking nanoscale light emitters},
journal = {Physics Today},
volume = {62},
number = {2},
pages = {34},
year = {2009},
doi = {10.1063/1.3086100}

}


@article{Rabouw,
author = {Rabouw, F. T. and van der Bok, J. C. and Spinicelli, P. and  Mahler, B. and Nasilowski, M. and Pedetti, S. and Dubertret, B. and Vanmaekelbergh, A.},
title = {{T}emporary {C}harge {C}arrier {S}eparation {D}ominates the {P}hotoluminescence {D}ecay {D}ynamics of {C}olloidal {C}d{S}e {N}anoplatelets},
journal = {Nano Lett.},
volume = {16},
number = {3},
pages = {2047-2053},
year = {2016},
doi = {10.1021/acs.nanolett.6b00053}

}




@article{Kulig,
 author = {Kulig, Marvin and Zipfel, Jonas and Nagler, Philipp and Blanter, Sofia and Sch\"uller, Christian and Korn, Tobias and Paradiso, Nicola and Glazov, Mikhail M. and Chernikov, Alexey}, 
 title = {{E}xciton {D}iffusion and {H}alo {E}ffects in {M}onolayer {S}emiconductors},
   journal = {Phys. Rev. Lett.},
  volume = {120},
  issue = {20},
  pages = {207401},
  numpages = {6},
  year = {2018},
    doi = {10.1103/PhysRevLett.120.207401}
 }



@article{Zipfel,
author = {Zipfel, Jonas and Kulig, Marvin and Perea-Caus\'{\i}n, Ra\"ul and Brem, Samuel and Ziegler, Jonas D. and Rosati, Roberto and Taniguchi, Takashi and Watanabe, Kenji and Glazov, Mikhail M. and Malic, Ermin and Chernikov, Alexey},
  title = {{E}xciton diffusion in monolayer semiconductors with suppressed disorder},
    journal = {Phys. Rev. B},
  volume = {101},
  issue = {11},
  pages = {115430},
  numpages = {20},
  year = {2020},
   doi = {10.1103/PhysRevB.101.115430}
}


@article{Glazov,
 author = {Glazov, M. M.}, 
 title = {{P}honon wind and drag of excitons in monolayer semiconductors},
   journal = {Phys. Rev. B},
  volume = {100},
  issue = {4},
  pages = {045426},
  numpages = {11},
  year = {2019},
   doi = {10.1103/PhysRevB.100.045426}
 }



@article{Olutas,
 author = {Olutas, M. and Guzelturk, B. and Kelestemur, Y. and Yeltik, A. and Delikanli, S. and Demir, H. V.}, 
 title = { {L}ateral {S}ize-{D}ependent {S}pontaneous and {S}timulated {E}mission {P}roperties in {C}olloidal {C}d{S}e {N}anoplatelets},
   journal = {ACS Nano},
  volume = {9},
  issue = {5},
  pages = {5041-5050},
    year = {2015},
   doi = {10.1021/acsnano.5b01927}
 }



@article{Rabouw_1,
 author = {Rabouw, Freddy T. and Kamp, Marko and van Dijk-Moes, Relinde J. A. and Gamelin, Daniel R. and Koenderink, A. Femius and Meijerink, Andries and Vanmaekelbergh, Daniel}, 
 title = { {D}elayed {E}xciton {E}mission and {I}ts {R}elation to {B}linking in {C}d{S}e {Q}uantum {D}ots},
   journal = {Nano Lett.},
  volume = {15},
  issue = {11},
  pages = {7718-7725},
    year = {2015},
   doi = {10.1021/acs.nanolett.5b03818}
 }



@article{Kunneman,
 author = {Kunneman, Lucas T. and Schins, Juleon M. and Pedetti, Silvia and Heuclin, Hadrien and Grozema, Ferdinand C. and Houtepen, Arjan J.  and Dubertret, Benoit}, 
 title = { {N}ature and {D}ecay {P}athways of {P}hotoexcited {S}tates in {C}d{S}e and {C}d{S}e/{C}d{S} {N}anoplatelets},
   journal = {Nano Lett.},
  volume = {14},
  issue = {12},
  pages = {7039-7045},
    year = {2014},
   doi = {10.1021/nl503406a}
 }


@article{Zamudio,
 author = {Del Pozo-Zamudio, O. and Schwarz, S. and Sich, M. and Akimov, I. A. and Bayer, M. and Schofield, R. C.  and Chekhovich,  E. A. and Robinson, B. J. and Kay, N. D. and  Kolosov, O.V. and Dmitriev, A. I. and  Lashkarev, G. V. and Borisenko, D. N. and Kolesnikov, N. N. and Tartakovskii, A. I.}, 
 title = { {P}hotoluminescence of two-dimensional {G}a{T}e and {G}a{S}e films},
   journal = { 2D Mater.},
  volume = {2},
  pages = {035010},
    year = {2015},
   doi = {10.1088/2053-1583/2/3/035010}
 }



@Article{Shornikova1,
author ={Shornikova, Elena V. and Biadala, Louis and Yakovlev, Dmitri R. and Sapega, Victor F. and Kusrayev, Yuri G. and Mitioglu, Anatolie A. and Ballottin, Mariana V. and Christianen, Peter C. M. and Belykh, Vasilii V. and Kochiev, Mikhail V. and Sibeldin, Nikolai N. and Golovatenko, Aleksandr A. and Rodina, Anna V. and Gippius, Nikolay A. and Kuntzmann, Alexis and Jiang, Ye and Nasilowski, Michel and Dubertret, Benoit and Bayer, Manfred},
title  ={{A}ddressing the exciton fine structure in colloidal nanocrystals: the case of {C}d{S}e nanoplatelets},
journal  ={Nanoscale},
year  ={2018},
volume  ={10},
issue  ={2},
pages  ={646-656},
doi  ={10.1039/C7NR07206F}
}


@Article{QLi,
author ={Li, Qiuyang and Lian, Tianquan},
title  ={{A}rea- and {T}hickness-{D}ependent {B}iexciton {A}uger {R}ecombination in {C}olloidal {C}d{S}e {N}anoplatelets: {B}reaking the {U}niversal {V}olume {S}caling {L}aw},
journal  ={Nano Lett.},
year  ={2017},
volume  ={17},
issue  ={5},
pages  ={3152-3158},
doi  ={10.1021/acs.nanolett.7b00587}
}



@Article{Wu,
author ={Li, Q. and Wu, K. and Chen,  J. and Chen, Z. and McBride, J. R. and Lian, T. },
title  ={{S}ize-{I}ndependent {E}xciton {L}ocalization {E}fficiency in {C}olloidal {C}d{S}e/{C}d{S} {C}ore/{C}rown {N}anosheet {T}ype-{I} {H}eterostructures},
journal  ={ACS Nano},
year  ={2016},
volume  ={10},
issue  ={3},
pages  ={3843-3851},
doi  ={10.1021/acsnano.6b00787}
}



@Article{NatComm2020,
author ={Seitz, Michael and Magdaleno, Alvaro J. and Alcazar-Cano, Nerea and Melendez, Marc and Lubbers, Tim J. and Walraven, Sanne W. and Pakdel, Sahar  and Prada, Elsa and  Delgado-Buscalioni, Rafael and Prins, Ferry},
title  ={{E}xciton diffusion in two-dimensional metal-halide perovskites},
journal  ={Nature Communications},
year  ={2020},
volume  ={11},
issue  ={1},
pages  ={2035},
doi  ={10.1038/s41467-020-15882-w}
}



@article{Irkhin2011,
 author = {Irkhin, Pavel and Biaggio, Ivan}, 
 title = {{D}irect {I}maging of {A}nisotropic {E}xciton {D}iffusion and {T}riplet {D}iffusion {L}ength in {R}ubrene {S}ingle {C}rystals},
   journal = {Phys. Rev. Lett.},
  volume = {107},
  issue = {1},
  pages = {017402},
  numpages = {4},
  year = {2011},
  doi = {10.1103/PhysRevLett.107.017402}
}


@article{MontrollWeiss,
author = {Montroll,Elliott W.  and Weiss,George H. },
title = {{R}andom {W}alks on {L}attices. {I}{I}},
journal = {Journal of Mathematical Physics},
volume = {6},
number = {2},
pages = {167-181},
year = {1965},
doi = {10.1063/1.1704269}
}


@article{ScherLax,
author = {Scher, H. and Lax, M.},
  title = {{S}tochastic {T}ransport in a {D}isordered {S}olid. {I}. {T}heory},
    journal = {Phys. Rev. B},
  volume = {7},
  issue = {10},
  pages = {4491--4502},
  numpages = {0},
  year = {1973},
  doi = {10.1103/PhysRevB.7.4491}
}



@article{ScherMontroll,
 author = {Scher, Harvey and Montroll, Elliott W.}, 
 title = {{A}nomalous transit-time dispersion in amorphous solids},
   journal = {Phys. Rev. B},
  volume = {12},
  issue = {6},
  pages = {2455--2477},
  numpages = {0},
  year = {1975},
  doi = {10.1103/PhysRevB.12.2455}
}



@BOOK{Hughes,
  title = { {R}andom {W}alks and {R}andom {E}nvironments, {V}ol. 1, {R}andom {W}alks},
  publisher = {Clarendon Press},
  year = {1995},
  author = {Hughes, B .D.},
  address = {Oxford, UK}
 
}



@article{bouchaud,
 author = {Jean-Philippe Bouchaud and Antoine Georges},
title = {{A}nomalous diffusion in disordered media: {S}tatistical mechanisms, models and physical applications},
journal = {Physics Reports},
volume = {195},
number = {4},
pages = {127 - 293},
year = {1990},
doi = {10.1016/0370-1573(90)90099-N},
}


@article{report2000,
author = {Ralf Metzler and Joseph Klafter},
title = {{T}he random walk's guide to anomalous diffusion: a fractional dynamics approach},
journal = {Physics Reports},
volume = {339},
number = {1},
pages = {1 - 77},
year = {2000},
doi = {10.1016/S0370-1573(00)00070-3}
}


@article{tiedje80,
author = {T. Tiedje and A. Rose},
title = {{A} physical interpretation of dispersive transport in disordered semiconductors},
journal = {Solid State Communications},
volume = {37},
number = {1},
pages = {49 - 52},
year = {1981},
doi = {10.1016/0038-1098(81)90886-3}
}



@MISC{GetData,
title = {{G}et{D}ata {G}raph {D}igitizer program}, url={http://getdata-graph-digitizer.com}
}



@article{Weidman,
author = {Weidman, Mark C. and Goodman, Aaron J. and Tisdale, William A.},
title = {{C}olloidal {H}alide {P}erovskite {N}anoplatelets: {A}n {E}xciting {N}ew {C}lass of {S}emiconductor {N}anomaterials},
journal = {Chem. Mater.},
volume = {29},
number = {12},
pages = {5019 - 5030},
year = {2017},
doi = {10.1021/acs.chemmater.7b01384}
}


@article{HavlinWeiss1990,
author = {Havlin, Shlomo and Weiss, George H.},
title = {{A} new class of long-tailed pausing time densities for the {C}{T}{R}{W}},
journal = {Journal of Statistical Physics},
volume = {58},
number = {5},
pages = {1267 - 1273},
year = {1990},
doi = {10.1007/BF01026577}
}


@article{chambers,
author = { J. M.   Chambers  and  C. L.   Mallows  and  B. W.   Stuck },
title = {{A} {M}ethod for {S}imulating {S}table {R}andom {V}ariables},
journal = {Journal of the American Statistical Association},
volume = {71},
number = {354},
pages = {340-344},
year  = {1976},
doi = {10.1080/01621459.1976.10480344},
}



@BOOK{Feller,
  title = { {A}n {I}ntroduction to {P}robability {T}heory and {I}ts {A}pplications, {V}ol. 2},
  publisher = {Edition, Wiley},
  year = {1991},
  author = {Feller, W.},
  address = {Cambridge, UK}
 
}


@BOOK{gnedenkokolmogorov,
  title = { {L}imit distributions for sums of independent random variables},
  publisher = {Addison-Wesley Mathematics Series},
  year = {1954},
  author = {Gnedenko, B. V. and Kolmogorov, A. N.},
  address = {Cambridge, UK}
 
}


@BOOK{samorodnitskii,
  title = { {S}table {N}on-{G}aussian {R}andom {P}rocesses: {S}tochastic {M}odels with {I}nfinite {V}ariance},
  publisher = {CRC Press},
  year = {1994},
  author = {Samorodnitsky, G. and Taqqu, M. S.}
}


@BOOK{VanKampen,
  title = { {S}tochastic {P}rocesses in {P}hysics and {C}hemistry},
  publisher = {Elsevier},
  year = {2007},
  author = {Van Kampen, N. G.}
}



























